Measurement of charm production cross-section and leptons from its semileptonic decay at RHIC

In this thesis, we present the measurements of $D^{0}\to K\pi$ at low $p_T$ ($p_T\leq2$ GeV/$c$) and non-photonic electron spectra ($0.9\leq p_T\leq5$ GeV/$c$) from $D^0$ semi-leptonic decay. In addition, we use a newly proposed technique to identify muons from charm decays at low $p_T$. The combination of all these three measurements stringently constrains the total charm production cross-section at mid-rapidity at RHIC. They also allow the extraction of the charmed hadron spectral shape and a study of possible charm radial flow in Au+Au collisions.

==> HFT.tex <==
\section{Heavy Flavor Tracker}


==> dilepton.tex <==
\section{Dileptons and J/$\psi$}


==> dplus.tex <==
\section{Charmed meson reconstruction}


==> effrates.tex <==
\section{Efficiencies and event rates estimation}


==> hfelossflow.tex <==
\section{Heavy flavor energy loss and collectivity}

As we discussed in the introduction chapter, the energy loss of
heavy quarks is considered as a unique tool to study the
interactions between heavy quarks and the medium created in the
heavy-ion collisions, and provide us important information of the
medium properties. Experimentally, the high \pt\ modifications of
heavy flavor hadron (D-mesons, B-mesons, {\em etc.}) yields are
expected to be the direct variables to reveal heavy quark energy
loss. But in current STAR experiment, it is very difficult to
topologically reconstruct D-mesons or B-mesons. And due to large
random combinatorial background, the same-/mixing-event method can
only provide the $D^0$ \pt\ spectrum below 2 \gevc\ with large
systematical uncertainties in minimum bias \AuAu\ collisions. In
central \AuAu\ collisions, the combinatorial background becomes
even larger, the signals are not good enough to extract useful
information. Due to small acceptance, direct measurement of heavy
flavor hadrons in PHENIX experiment becomes even harder.
Nevertheless, the measurements of single electron from heavy quark
decays were used as the indirect substitute.

The single electron strong suppression, similar to light hadrons,
was observed in recent measurements. Fig.~\ref{eraa} shows the
nuclear modification factor of single muons (open crosses) and
electrons (solid squares), \RAA\, as a function of \pt\ measured
from STAR TPC+TOF detector. The \RAA\ are obtained using \dAu\ fit
curve as reference, which has been discussed in previous section.
The PHENIX result and STAR EMC result, \raa\, which use electron
spectra measured in \pp\ collisions as references, are shown as
open circles and solid circles for comparison. Within errors,
these results are consistent in different experiments. The \RAA\
may show some Cronin effect due to enhancement in \dAu\ collisions
relative to \pp\ collisions $R_{dAu}>1$. But this effect is not
significant compared to huge error bars.

\bf \centering\mbox{
\includegraphics[width=0.6\textwidth]{plots/RAAe_1.eps}}
\caption[Single electron nuclear modification factors.]{Nuclear
modification factors of single electrons as a function of \pt.}
\label{eraa} \ef

Here still exists some puzzles: how can the behavior of heavy
flavor decay electrons reflect heavy quarks? Is the medium also
opaque to heavy quarks? What is the contribution of bottom in
single electron measurements?

Fig.~\ref{Dptvsept} shows the 2D-scattering plot of D-meson \pt(D)
versus decay electron \pt(e) from form factor decay. The inserted
small panel shows the D-meson \pt(D) distributions when select
electron at $1.45<p_T(e)<1.55$ \gevc. $\sim$ 92\% yields of
D-meson are from $1<p_T(D)<4$ \gevc. This indicates that the \pt\
correlation between single electrons and their parent D-mesons is
weak.

\bf \centering\mbox{
\includegraphics[width=0.6\textwidth]{plots/Dptvsept.eps}}
\caption[2D-scattering plot of D-meson \pt\ versus electron
\pt.]{2D-scattering plot of D-meson \pt(D) versus electron \pt(e)
from form factor decay.} \label{Dptvsept} \ef

On the other hand, due to large mass and small radiative angle,
heavy quarks are predicted to lose less energy than light quarks
via only gluon radiation -- the "dead cone" effect. Many
theoretical calculations tried to explain the single electron
strong suppression observed in experiments. A collisional
(elastic) energy loss has been proposed to be taken into account
for heavy quark energy loss calculations.

\bf \centering\mbox{
\includegraphics[width=0.6\textwidth]{plots/raa_1.eps}}
\caption[Theoretical calculations for single electron \raa\
compared to data.]{Theoretical calculations for single electron
\raa\ compared to data.} \label{raa1} \ef

Fig.~\ref{raa1} shows some recent theoretical calculations for
single electron \raa\ from heavy flavor semi-leptonic decays. The
DGLV radiative energy loss via few hard scatterings with initial
gluon density $dN_g/dy=1000$ predicts significantly less
suppression than data, shown as curve 1. The curve drops
dramatically after including collisional energy loss, shown as
curve 2, but still predicts less suppression than observed. Curve
3, which has a good agreement with data, is from the calculation
of heavy quark energy loss via elastic scattering mediated by
resonance excitations of D- and B- mesons and LO pQCD gluon
exchange, and including heavy-light quark-coalescence at
hadronization. The double-curve indicate the uncertainties from
the calculation assuming the D- and B- resonance width
$\Gamma=0.4-0.75$ \gev. Curve 4 shows the calculation of single
electron suppression from collisional dissociation of heavy mesons
in QGP by deriving heavy meson survival and dissociation
probability from the collisional broadening of their light cone
wave function. The double-curve indicate the uncertainties from
tuning the typical value of $\xi\sim2-3$. This calculation also
shows consistent suppression with data. Curve 5 is for single
electron only from D-meson decays with only radiative energy loss
from BDMPS calculations. Curve 6, which is the same calcuation as
curve 5 but including electron from B-meson decays and assuming
the transport coefficient $\hat{q}=14 GeV^2/fm$. Both these two
curves from BDMPS calculations agree with data.

Many assumptions still remain for theoretical calculations. And
many different processes turn out the similar results, which can
describe data within large errors. The heavy quark energy loss
mechanism is still a puzzle from current single electron
experiments.

Theoretical calculations have shown that interactions between the
surrounding partons in the medium and heavy quarks could change
the measurable kinematics\cite{teaney,rapp,dd1}, and could boost
the radial and elliptic flow resulting in a different heavy quark
\pt\ spectrum shape. Due to their heavy mass and partonic density
gradient, such a heavy quark may acquire flow from the sufficient
interactions with the constituents of a dense medium in analog to
Brownian motion. Fig.~\cite{hfcollectivity} shows the picture that
heavy quarks participate in collective motion. We expect that
bottom quark has small collective velocity due to its extremely
heavy mass. Its decoupling from medium also depends on the
cross-section of the interaction and medium density. Therefore,
the measurement of heavy flavor flow and freeze-out properties is
vital to test light flavor thermalization and the partonic density
in the early stage of heavy ion collisions
\cite{xu2,teaney,batsouli}.

\bf \centering \bmn[c]{0.47\textwidth} \centering
\includegraphics[width=0.95\textwidth]{plots/cquark.eps}
\emn%
\bmn[c]{0.5\textwidth} \centering
\includegraphics[width=0.95\textwidth]{plots/bquark.eps}
\emn%
\caption[heavy quark collective motion]{Heavy quark collective
motion.} \label{hfcollectivity} \ef


==> hftsimu.tex <==
\chapter{Charm-hadron reconstruction with Heavy Flavor Tracker}


\input{HFT}
\input{dplus}
\input{lambdac}
\input{effrates}


==> lambdac.tex <==
\section{Charmed baryon reconstruction}


==> outlook.tex <==
\chapter{Detector upgrades and outlook}

\input{upgrade}
\input{directc}
\input{isobc}
%\input{dilepton}
%\subsection{Direct measurements of charmed hadrons}
%\subsection{}
%\subsection{Reconstruction efficiencies and event rates estimation}

